What the Fix? A Study of ASATs Rule Documentation

Automatic Static Analysis Tools (ASATs) are widely used by software developers to diffuse and enforce coding practices. Yet, we know little about the documentation of ASATs, despite it being critical to learn about the coding practices in the first place. We shed light on this through several contributions. First, we analyze the documentation of more than 100 rules of 16 ASATs for multiple programming languages, and distill a taxonomy of the purposes of the documentation-What triggers a rule; Why it is important; and how to Fix an issue-and its types of contents. Then, we conduct a survey to assess the effectiveness of the documentation in terms of its goals and types of content. We highlight opportunities for improvement in ASAT documentation. In particular, we find that the Why purpose is missing in half of the rules we survey; moreover, when the Why is present, it is more likely to have quality issues than the What and the Fix.

==> Sections/Background.tex <==
\section{Background}
\label{sec:background}

\subsection{Coding practices}
\label{subsec:coding_practices}

This practice is general and may apply to all software projects, but the majority of practices are language or technology dependent.
An example of standard practice in JavaScript is using the \emph{let} keyword instead of \emph{var} to declare a non-constant variable.

A practice is not set in stone, as languages and technologies are evolving, it also applies to coding practices.

Another essential source comes from the developer's own journey.
Exchanging or seeing the code of other peers allows one to discover new practices and adapt own accordingly.

\subsection{Practices diffusion}
\label{subsec:practices_diffusion}

To ensure they will be applied, having company practices readily available is essential, especially for newcomers.
There are many mediums available for developers to broadcast and access them.
One practical approach is using wikis, where the practices are described in natural language with code examples.
Tools like Notion or Miro ease this collaboration work~\cite{jackson_collaboration_2022}.
In a similar approach, Stack Overflow also proposes a solution for the teams to help them share their knowledge.
We also find some processes in the modern development workflow allowing exchange and transfer between developers, such as during coding dojos~\cite{sato_coding_2008} or code reviews~\cite{bacchelli_expectations_2013}.

Even if practices are accessible and well described, there is no insurance that developers will apply, especially if there are many of them.
It is easy to forget one or simply never encounter it.
To help to track their adoption, tools like linters have been developed.

\subsection{Linters}
\label{subsec:linters}

Talks about: a rule is a practice implementation in a specific linter.
Article on linters' benefice to learn new language specificity~\cite{tomasdottir_why_2017}
Technically, it parses the code to create an abstract syntax tree representation and uses a visitor to validate each node's features.
In \Cref{subsec:coding_practices}, we introduce a practice advising to avoid the use of the \emph{var} in JavaScript.
The linter ESLint\footnote{\url{https://eslint.org}} offers the possibility to warn automatically this defect using the rule \emph{no-var}\footnote{\url{https://eslint.org/docs/latest/rules/no-var}}.


==> Sections/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

